SenseFlow: A Physics-Informed and Self-Ensembling Iterative Framework for Power Flow Estimation

Power flow estimation plays a vital role in ensuring the stability and reliability of electrical power systems, particularly in the context of growing network complexities and renewable energy integration. However, existing studies often fail to adequately address the unique characteristics of power systems, such as the sparsity of network connections and the critical importance of the unique Slack node, which poses significant challenges in achieving high-accuracy estimations. In this paper, we present SenseFlow, a novel physics-informed and self-ensembling iterative framework that integrates two main designs, the Physics-Informed Power Flow Network (FlowNet) and Self-Ensembling Iterative Estimation (SeIter), to carefully address the unique properties of the power system and thereby enhance the power flow estimation. Specifically, SenseFlow enforces the FlowNet to gradually predict high-precision voltage magnitudes and phase angles through the iterative SeIter process. On the one hand, FlowNet employs the Virtual Node Attention and Slack-Gated Feed-Forward modules to facilitate efficient global-local communication in the face of network sparsity and amplify the influence of the Slack node on angle predictions, respectively. On the other hand, SeIter maintains an exponential moving average of FlowNet's parameters to create a robust ensemble model that refines power state predictions throughout the iterative fitting process. Experimental results demonstrate that SenseFlow outperforms existing methods, providing a promising solution for high-accuracy power flow estimation across diverse grid configurations.

==> tables/abl_weights.tex <==

\begin{table}[t]
\caption{Effects of the weight $\lambda$ on the equation loss $\mathcal{L}_{equ}$. We set $\lambda$ as 0.1 by default.}
\label{tab:abl:equ}
% \vskip 0.15in
\begin{center}
% \resizebox{0.99\linewidth}{!}{
\begin{tabular}{ccccccc}
\toprule
% \multirow{2}{*}{$\lambda$} & \multicolumn{5}{c}{IEEE-Bus39} & \multicolumn{5}{c}{IEEE-Bus118} \\ 
%   % \cline{2-6} \cline{7-11}
%    \cmidrule(lr){2-6} \cmidrule(lr){7-11}
$\lambda$ & 0.0 & 0.05 & 0.10 & 0.15 & 0.20& 0.25 \\
\midrule
PQ$_\text{Vm}$ & 0.00099400  & 0.00083139  & 0.00078161   & 0.00118891  & \textbf{0.00075882}  & 0.00111757  \\
PQ$_\text{Va}$ & 0.01137573  & 0.00768562  & 0.00608600   & 0.00752592  & \textbf{0.00590381}  & 0.00866294 \\
PV$_\text{Va}$ & 0.01234842  & 0.00835177  & \textbf{0.00609802}   & 0.00805090  & 0.00646078  & 0.00960786  \\
\bottomrule
\end{tabular}
% }
\end{center}
% \vskip -0.1in
\end{table}

\begin{table}[ht]
\caption{Power flow estimation on IEEE 1354pegase.}
\label{tab:abl:1k3}
\begin{center}
% \resizebox{0.99\linewidth}{!}{
\begin{tabular}{lccccc}
\toprule
 & PQ$_\text{Vm}$ & PQ$_\text{Va}$ & PV$_\text{Va}$ \\
\midrule
PowerflowNet [21] with 2k-ep     & 0.00082930 & 0.02937557 & 0.02814063 \\
Senseflow with 100-ep     & 0.00196035 & 0.03509841 & 0.03051907 \\
Senseflow with 500-ep     & \textbf{0.00013276} & \textbf{0.00077648} & \textbf{0.00071715}  \\
\bottomrule
\end{tabular}
% }
\end{center}
\end{table}

